Development of a Human-Robot Interaction Platform for Dual-Arm Robots Based on ROS and Multimodal Artificial Intelligence

In this paper, we propose the development of an interactive platform between humans and a dual-arm robotic system based on the Robot Operating System (ROS) and a multimodal artificial intelligence model. Our proposed platform consists of two main components: a dual-arm robotic hardware system and software that includes image processing tasks and natural language processing using a 3D camera and embedded computing. First, we designed and developed a dual-arm robotic system with a positional accuracy of less than 2 cm, capable of operating independently, performing industrial and service tasks while simultaneously simulating and modeling the robot in the ROS environment. Second, artificial intelligence models for image processing are integrated to execute object picking and classification tasks with an accuracy of over 90%. Finally, we developed remote control software using voice commands through a natural language processing model. Experimental results demonstrate the accuracy of the multimodal artificial intelligence model and the flexibility of the dual-arm robotic system in interactive human environments.

==> vncaps.tex <==
% Copyright 2000-2006 Werner Lemberg <wl@gnu.org> and
%                     Han The Thanh <hanthethanh@gmx.net>.
% This file is part of vntex.  License: LPPL, version 1.3 or newer,
% according to http://www.latex-project.org/lppl.txt

\ifx\ProvidesFile\undefined \else
  \ProvidesFile{vncaps.tex}[2006/06/07 v1.1 Captions in Vietnamese]  
\fi
 
% Vietnamese captions; edit them in viscii/tcvn/utf8, then use
% `vntovn viscii vntex' or a similar command to convert to vntex.
%
% History
%
% ????/??/??:
%     Split off captions from vietnam.ldf.
%     Add \captionsenglish, \dateUSenglish, and \dateenglish.
%
% 2005/04/21:
%     Add copyright message.
%     Don't use `{}' but a space after macros which don't have arguments.
%
% 2006/06/07:
%     Fix bug in \indexname.  Add version number.

\ifx\providecommand \undefined
  \let\providecommand \def
\fi

\providecommand\captionsvietnam{% 
  \def\prefacename{L\`\ohorn i n\'oi \dj\`\acircumflex u}%
%  \def\refname{T\`ai li\d\ecircumflex u}%
  \def\Acknowledgmentname{L\`\ohorn i c\h{a}m \ohorn n}%
  \def\refname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
%  \def\abstractname{T\'om t\'\abreve t n\d\ocircumflex i dung}
  \def\abstractname{T\'om t\'\abreve t}
  \def\IEEEkeywordsname{T\`\uhorn \, kh\'oa}
  \def\bibname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
  \def\chaptername{Ch\uhorn \ohorn ng}%
  \def\appendixname{Ph\d{u} l\d{u}c}%
  \def\contentsname{M\d{u}c l\d{u}c}%
  \def\listfigurename{Danh s\'ach h\`inh v\~e}%
  \def\listtablename{Danh s\'ach b\h{a}ng}%
  \def\indexname{Ch\h{i} m\d{u}c}% 
  \def\figurename{H\`inh}%
  \def\tablename{B\h{a}ng}%
  \def\partname{Ph\`\acircumflex n}%
  \def\pagename{Trang}%
  \def\headpagename{Trang}%
  \def\seename{Xem}%
  \def\alsoname{Xem th\ecircumflex m}%
  \def\enclname{K\`em theo}%
  \def\ccname{C\`ung g\h\uhorn i}%
  \def\headtoname{G\h\uhorn i}%
  \def\proofname{Ch\'\uhorn ng minh}}

\providecommand\datevietnam{%
  \def\today{%
    Ng\`ay \number\day\space
    th\'ang \number\month\space
    n\abreve m \number\year}}

\providecommand\captionsenglish{%
  \def\prefacename{Preface}%
  \def\refname{References}%
  \def\abstractname{Abstract}%
  \def\bibname{Bibliography}%
  \def\chaptername{Chapter}%
  \def\appendixname{Appendix}%
  \def\contentsname{Contents}%
  \def\listfigurename{List of Figures}%
  \def\listtablename{List of Tables}%
  \def\indexname{Index}%
  \def\figurename{Figure}%
  \def\tablename{Table}%
  \def\partname{Part}%
  \def\enclname{encl}%
  \def\ccname{cc}%
  \def\headtoname{To}%
  \def\pagename{Page}%
  \def\headpagename{Page}%
  \def\prefacename{Preface}%
  \def\seename{see}%
  \def\alsoname{see also}}

\providecommand\dateenglish{%
  \def\today{%
    \ifcase\day\or 1st\or 2nd\or 3rd\or 4th\or 5th\or 6th\or 7th\or
    8th\or 9th\or 10th\or 11th\or 12th\or 13th\or 14th\or 15th\or
    16th\or 17th\or 18th\or 19th\or 20th\or 21st\or 22nd\or 23rd\or
    24th\or 25th\or 26th\or 27th\or 28th\or 29th\or 30th\or 31st\fi
    ~\ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space
    \number\year}}

\providecommand\dateUSenglish{%
  \def\today{%
    \ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space\number\day, \number\year}}

\endinput

% end of vncaps.tex

